AI-Aided Integrated Terrestrial and Non-Terrestrial 6G Solutions for Sustainable Maritime Networking

The maritime industry is experiencing a technological revolution that affects shipbuilding, operation of both seagoing and inland vessels, cargo management, and working practices in harbors. This ongoing transformation is driven by the ambition to make the ecosystem more sustainable and cost-efficient. Digitalization and automation help achieve these goals by transforming shipping and cruising into a much more cost- and energy-efficient, and decarbonized industry segment. The key enablers in these processes are always-available connectivity and content delivery services, which can not only aid shipping companies in improving their operational efficiency and reducing carbon emissions but also contribute to enhanced crew welfare and passenger experience. Due to recent advancements in integrating high-capacity and ultra-reliable terrestrial and non-terrestrial networking technologies, ubiquitous maritime connectivity is becoming a reality. To cope with the increased complexity of managing these integrated systems, this article advocates the use of artificial intelligence and machine learning-based approaches to meet the service requirements and energy efficiency targets in various maritime communications scenarios.

==> Fig3.tex <==
\begin{tikzpicture}

\pgfplotsset{every tick label/.append style={font=\scriptsize}}

\begin{axis}[
	%x tick label style={/pgf/number format/1000 sep=},
	width=\columnwidth,
    height=0.76\columnwidth,
	x label style={font=\scriptsize},
    y label style={font=\scriptsize},
	ylabel = {Energy efficiency (Mbit/Joule)},
	xlabel = {Maximum capacity share},
	%enlargelimits = 0.15,
	legend style={font=\scriptsize, anchor=north east, at={(0.27,0.97)}},
	ymax = 14,
	ybar,
	bar width=7pt,
	%xmajorgrids,
    ymajorgrids,
]

\addplot[color=green,fill=green!70!white, postaction={pattern=north west lines}]table[row sep=crcr]{
0.1	6.5029732814641\\
0.2	7.83949872186546\\
0.3	12.2362931497857\\
0.4	13.2065743169330\\
0.5	13.8565261692997\\
    };

\addplot[color=orange,fill=orange!70!white, postaction={pattern=north east lines}]table[row sep=crcr]{
0.1 4.58317827831103\\
0.2 5.66203333723438\\
0.3 9.39285679314566\\
0.4 9.30956072351421\\
0.5 12.1536893992592\\
	};

\legend{DNN-aided, Baseline}

\end{axis}

\end{tikzpicture}

==> Fig4.tex <==
\begin{tikzpicture}

\pgfplotsset{every tick label/.append style={font=\scriptsize}}
%\tikzstyle{dashed}= [dash pattern=on 7.5*0.8*0.8pt off 7.5*0.4*0.8pt]

\begin{axis}[%
    %x tick label style={/pgf/number format/1000 sep=}
    axis y line*=left,
    xmin=0,
    xmax=2,
    x label style={font=\small},
    y label style={font=\small,color=orange},
    xlabel = {User density ($\textup{users/m}^2$)},
    %xtick = {0,0.5,1,1.5,2},
    %xticklabels = {0,$0.5 \cdot 10^6$,$1\cdot 10^6$,$1.5\cdot 10^6$,$2\cdot 10^6$},
    ymin=0,
    ymax=3,
    ylabel={Packet delay (s)},
    xmajorgrids,
    ymajorgrids,
    legend style={font=\scriptsize, at={(0.5,1)}, anchor=north east, legend cell align=left, align=left, draw=white!15!black}
],

\addplot [color=orange, dashed, mark=square, mark options={solid}, line width=0.8pt]
  table[row sep=crcr]{
0 0\\
0.2	0.286291\\
0.4	0.551094\\
0.6	0.807503\\
0.8	1.13558\\
1	1.44828\\
1.2	1.59867\\
1.4	1.8146\\
1.6	2.01709\\
1.8	2.14754\\
2	2.34182\\
};
\addlegendentry{Baseline};

\addplot [color=orange, mark=square, line width=0.8pt]
  table[row sep=crcr]{
0 0\\
0.2	0.152224\\
0.4	0.289077\\
0.6	0.423391\\
0.8	0.555136\\
1	0.684377\\
1.2	0.811081\\
1.4	0.935001\\
1.6	1.05655\\
1.8	1.16956\\
2	1.24082\\
};
\addlegendentry{LSTM-aided scheduling};
\end{axis};

\begin{axis}[
    axis y line*=right,
    y label style={font=\small, color=green},
    ylabel={Energy efficiency (Mbit/Joule)},
    ymin=0,
    ymax=12,
    xmin=0,
    xmax=2,
    axis x line = none,
    legend style={font=\scriptsize, at={(1,1)}, anchor=north east, legend cell align=left, align=left, draw=white!15!black}
]

\addplot [color=green, mark=triangle, line width=0.8pt]
  table[row sep=crcr]{
0	0\\
0.2	6.98795\\
0.4	7.42245\\
0.6	8.36109\\
0.8	8.36896\\
1	8.3815\\
1.2	8.38256\\
1.4	8.37625\\
1.6	8.37457\\
1.8	8.37235\\
2	8.36109\\
};
\addlegendentry{LSTM-aided scheduling}

\addplot [color=green, mark=triangle, mark options={solid}, dashed, line width=0.8pt]
  table[row sep=crcr]{
0 0\\
0.2 3.53298\\
0.4 3.96748\\
0.6 4.23583\\
0.8 4.23597\\
1 4.23869\\
1.2 4.3957\\
1.4 4.23788\\
1.6 4.23347\\
1.8 4.23294\\
2 4.23158\\
};
\addlegendentry{Baseline};

\end{axis};

\end{tikzpicture}


==> IEEE NetMag 2021 - arxiv/Fig3.tex <==
\begin{tikzpicture}

\pgfplotsset{every tick label/.append style={font=\scriptsize}}

\begin{axis}[
	%x tick label style={/pgf/number format/1000 sep=},
	width=\columnwidth,
    height=0.76\columnwidth,
	x label style={font=\scriptsize},
    y label style={font=\scriptsize},
	ylabel = {Energy efficiency (Mbit/Joule)},
	xlabel = {Maximum capacity share},
	%enlargelimits = 0.15,
	legend style={font=\scriptsize, anchor=north east, at={(0.27,0.97)}},
	ymax = 14,
	ybar,
	bar width=7pt,
	%xmajorgrids,
    ymajorgrids,
]

\addplot[color=green,fill=green!70!white, postaction={pattern=north west lines}]table[row sep=crcr]{
0.1	6.5029732814641\\
0.2	7.83949872186546\\
0.3	12.2362931497857\\
0.4	13.2065743169330\\
0.5	13.8565261692997\\
    };

\addplot[color=orange,fill=orange!70!white, postaction={pattern=north east lines}]table[row sep=crcr]{
0.1 4.58317827831103\\
0.2 5.66203333723438\\
0.3 9.39285679314566\\
0.4 9.30956072351421\\
0.5 12.1536893992592\\
	};

\legend{DNN-aided, Baseline}

\end{axis}

\end{tikzpicture}

==> IEEE NetMag 2021 - arxiv/Fig4.tex <==
\begin{tikzpicture}

\pgfplotsset{every tick label/.append style={font=\scriptsize}}
%\tikzstyle{dashed}= [dash pattern=on 7.5*0.8*0.8pt off 7.5*0.4*0.8pt]

\begin{axis}[%
    %x tick label style={/pgf/number format/1000 sep=}
    axis y line*=left,
    xmin=0,
    xmax=2,
    x label style={font=\small},
    y label style={font=\small,color=orange},
    xlabel = {User density ($\textup{users/m}^2$)},
    %xtick = {0,0.5,1,1.5,2},
    %xticklabels = {0,$0.5 \cdot 10^6$,$1\cdot 10^6$,$1.5\cdot 10^6$,$2\cdot 10^6$},
    ymin=0,
    ymax=3,
    ylabel={Packet delay (s)},
    xmajorgrids,
    ymajorgrids,
    legend style={font=\scriptsize, at={(0.5,1)}, anchor=north east, legend cell align=left, align=left, draw=white!15!black}
],

\addplot [color=orange, dashed, mark=square, mark options={solid}, line width=0.8pt]
  table[row sep=crcr]{
0 0\\
0.2	0.286291\\
0.4	0.551094\\
0.6	0.807503\\
0.8	1.13558\\
1	1.44828\\
1.2	1.59867\\
1.4	1.8146\\
1.6	2.01709\\
1.8	2.14754\\
2	2.34182\\
};
\addlegendentry{Baseline};

\addplot [color=orange, mark=square, line width=0.8pt]
  table[row sep=crcr]{
0 0\\
0.2	0.152224\\
0.4	0.289077\\
0.6	0.423391\\
0.8	0.555136\\
1	0.684377\\
1.2	0.811081\\
1.4	0.935001\\
1.6	1.05655\\
1.8	1.16956\\
2	1.24082\\
};
\addlegendentry{LSTM-aided scheduling};
\end{axis};

\begin{axis}[
    axis y line*=right,
    y label style={font=\small, color=green},
    ylabel={Energy efficiency (Mbit/Joule)},
    ymin=0,
    ymax=12,
    xmin=0,
    xmax=2,
    axis x line = none,
    legend style={font=\scriptsize, at={(1,1)}, anchor=north east, legend cell align=left, align=left, draw=white!15!black}
]

\addplot [color=green, mark=triangle, line width=0.8pt]
  table[row sep=crcr]{
0	0\\
0.2	6.98795\\
0.4	7.42245\\
0.6	8.36109\\
0.8	8.36896\\
1	8.3815\\
1.2	8.38256\\
1.4	8.37625\\
1.6	8.37457\\
1.8	8.37235\\
2	8.36109\\
};
\addlegendentry{LSTM-aided scheduling}

\addplot [color=green, mark=triangle, mark options={solid}, dashed, line width=0.8pt]
  table[row sep=crcr]{
0 0\\
0.2 3.53298\\
0.4 3.96748\\
0.6 4.23583\\
0.8 4.23597\\
1 4.23869\\
1.2 4.3957\\
1.4 4.23788\\
1.6 4.23347\\
1.8 4.23294\\
2 4.23158\\
};
\addlegendentry{Baseline};

\end{axis};

\end{tikzpicture}

